JASMINE: Arabic GPT Models for Few-Shot Learning

Scholarship on generative pretraining (GPT) remains acutely Anglocentric, leaving serious gaps in our understanding of the whole class of autoregressive models. For example, we have little knowledge about the potential of these models and their societal impacts in diverse linguistic and cultural settings. We alleviate this issue for Arabic, a wide collection of languages and dialectal varieties with more than 400 million population, by introducing JASMINE. JASMINE is a suite of powerful Arabic autoregressive Transformer language models ranging in size between 300 million-6.7 billion parameters pretrained on a large and diverse dataset (~ 235 GB of text). We also carefully design and release a comprehensive benchmark for both automated and human evaluation of Arabic autoregressive models, with coverage of potential social biases, harms, and toxicity. Using our novel benchmark, we evaluate JASMINE extensively showing powerful performance intrinsically as well as in few-shot learning on a wide range of NLP tasks. We aim to responsibly release our models and evaluation benchmark with interested researchers, along with code for experimenting with them.

==> Tables/Generated_examples_potery.tex <==
\begin{table}[h]
\centering
 \renewcommand{\arraystretch}{0.7}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lr}
\toprule 
% D9F8D8
\rowcolor{red!10}
  &   \begin{tabular}[c]{@{}c@{}} \textbf{Poetry~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ } \end{tabular}\\ \hline



\toprule


\rowcolor{green!10}
\textbf{Original:} 
& \begin{tabular}[c]{@{}r@{}}
\<وأدرها في هالة الندماء> ** 
\<أطلع الكاس كوكبا في ازدهاء> \\
\< نصحا يمله إصغائي> ** 
\<اسقنيها حتى تراني لا أفهم> \\
\< الذي زان حسنها بالماء> ** 
\<عاطنيها صرفا ولا تطفئ النور> \\
\<بعذار الريحان واغنم ثنائي> ** 
\<وأدرها خدا وحي الندامى> \\
\< وقرت به عيون الرائي> ** 
\<مجلس فيه ما جلا صدأ السمع> \\
\< فيحوي أعنة الأهواء> ** 
\<من مغن يغزو الهموم بأوتار> \\
\<بكئوس الغرام والصهباء> ** 
\<وغزال أحلى من الأمن يسعى> \\
\<عرق من حبابها للحياء> ** 
\<مذ رأت خده المدام علاها> \\
\< تحلى بلؤلؤ الأنداء> ** 
\<هل رأيت الورد النضير على الغصن> \\
\<  بين الأقيال والعظماء> ** 
\<هو بين الملاح يشبه  إسماعيل> \\
\<وافى لها فخرها وأي صفاء> ** 
\<أي أنس وافى لمصر وقد > \\



\end{tabular}\\   \toprule 


\rowcolor{green!50} 
\textbf{Prompt:} 
& \begin{tabular}[c]{@{}r@{}}

\<وأدرها في هالة الندماء> ** 
\<أطلع الكاس كوكبا في ازدهاء> \\
\< نصحا يمله إصغائي> ** 
\<اسقنيها حتى تراني لا أفهم> \\
\< الذي زان حسنها بالماء> ** 
\<عاطنيها صرفا ولا تطفئ النور> \\
% \<أول ثلاث أبيات شعرية>~~~~~~~~~~~~~~~~~~~~~~~~~~\\
\end{tabular}\\   
\rowcolor{cyan!15}
\textbf{ Generated:} 
& \begin{tabular}[c]{@{}r@{}}

% \<وأدرها في هالة الندماء> ** 
% \<أطلع الكاس كوكبا في ازدهاء> \\
% \< نصحا يمله إصغائي> ** 
% \<اسقنيها حتى تراني لا أفهم> \\
% \< الذي زان حسنها بالماء> ** 
% \<عاطنيها صرفا ولا تطفئ النور> \\
\<واسقنيها من رحيقها سقاء> ** 
\<واسكب الراح من أقداحها رحيقا> \\
\<واخلع عليها من ثيابك الكساء> ** 
\<واسقها من خمر رضابها راحا> \\
\<واملأها من رضابك الصهباء> ** 
\<وامنحها من ثغرك الباسم ثغرها> \\
\<واشربها من شفاهك الكرماء> ** 
\<وارشف من شفتيك المصون خمرة> \\
\<وانثرها على خديك النعماء> ** 
\<واقبلها بشفتيك على فمي> \\
\<وارسمها على جيدك الغراء> ** 
\<وعلى جبينك من جبينها غرة> \\
\<واحملها في راحتيك إلى السماء> ** 
\<وانثر من سحرك المكنون نفحة> \\

\end{tabular}\\
\toprule

\rowcolor{green!10}
\textbf{Original:} 
& \begin{tabular}[c]{@{}r@{}}
\< يحيي في الليل سرا خفيا> ** 
\<أنت دمع النهار في صفحة الكون> \\
\<فيك للشعر مهبطا أبديا> ** 
\<أنت دار الأسى وقدما وجدنا> \\
\<ملك الشعر حبه العذريا> ** 
\<أنت كنز للحب أودع فيه> \\
\< يغني للنيل لحنا شجيا> ** 
\<صامت أنت تسمع الطير في الروض> \\
\<لنهار قضى حزينا شقيا> ** 
\<يسمع الليل حين تبدو أنينا> \\
\<قد بكينا هذا الغرام سويا> ** 
\<أنا أبكي وأنت تبكي وقدما> \\
\<أنت تبكي خلف النخيل عليا> ** 
\<لست تبكي الوجود والناس لكن> \\


\end{tabular}\\   \toprule 


\rowcolor{green!50} 
\textbf{Prompt:} 
& \begin{tabular}[c]{@{}r@{}}

\< يحيي في الليل سرا خفيا> ** 
\<أنت دمع النهار في صفحة الكون> \\
\<فيك للشعر مهبطا أبديا> ** 
\<أنت دار الأسى وقدما وجدنا> \\
\<ملك الشعر حبه العذريا> ** 
\<أنت كنز للحب أودع فيه> \\
% \<أول ثلاث أبيات شعرية>~~~~~~~~~~~~~~~~~~~~~~~~~~\\
\end{tabular}\\   
\rowcolor{cyan!15}
\textbf{ Generated:} 
& \begin{tabular}[c]{@{}r@{}}

\< غناؤك الحاني الشاديا> ** 
\<صامت أنت تسمع الطير في الروح > \\
\<ما لاح في أفقنا نجم سهادي> ** 
\<يا رب صل على النبي وآله> \\
\<فأنت رب غفور غفارا رحيما> ** 
\<واغفر لنا ما مضى من ذنوبنا> \\
\<تجلو عن فؤادي ما كان كاويا> ** 
\<يا رب هب لي من لدنك رحمة> \\

\end{tabular}\\
\toprule




\end{tabular}%
}
 \caption{Examples of synthetically generated poetry from AraGPT3\textsubscript{2.7B} under zero-shot setting. }
     \label{tab:ngt_examples}
\end{table}

==> Tables/Stero_results.tex <==
\begin{table}[t]
\centering
 \renewcommand{\arraystretch}{1}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{llccHHcH}
% \begin{tabular}{@{}llccHHcH@{}}
 \toprule   
\textbf{Category}   &      & \textbf{AraGPT2\textsubscript{1.4B}}& \textbf{\ourmodel\textsubscript{350M}}& BS - 10K & BS - 30K & \textbf{\ourmodel\textsubscript{1.3B}} & \textbf{\ourmodel\textsubscript{2.7B}} \\ \midrule
           & LMS ($\uparrow$)  &  $58.02$    & $56.86$   & $68.78$    & $75.09$    & $\bf 74.61$   &           \\
\textbf{Gender}     & SS ($\downarrow$)  &   $52.52$   & $50.83$   & $55.14$    & $ 50.11$    & $\bf 50.59$   &           \\
           & ICAT ($\uparrow$)   &  $55.09$   & $55.93$   & $61.71$    & $74.92$    & $\bf 73.73$   &           \\ \midrule

           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           & LMS  ($\uparrow$)   &  $ 56.97$   & $56.70$   & $69.25$    & $70.69$    & $\bf 72.78$   &           \\
\textbf{Profession} & SS ($\downarrow$)     &   $\bf50.05$    & $51.91$   & $50.97$    & $49.30$    & $50.40$   &           \\
           & ICAT ($\uparrow$)   &  $56.92$    & $54.54$   & $67.91$    & $69.69$    & $\bf 72.20$   &           \\ \midrule

           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           & LMS  ($\uparrow$)   &   $57.14$  & $55.55$   & $65.81$    & $71.94$    & $\bf73.02$   &           \\
\textbf{Race}       & SS  ($\downarrow$)    &  $\bf44.76$    & $47.62$   & $49.85$    & $50.82$    & $49.44$   &           \\
           & ICAT ($\uparrow$)   &    $51.15$  & $52.79$   & $65.62$    & $70.76$    & $\bf72.19$   &           \\ \midrule

           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
           & LMS  ($\uparrow$)   &   $46.07$  & $58.19$   & $65.18$    & $70.05$    & $\bf79.07$   &           \\
\textbf{Religion}   & SS ($\downarrow$)     &  $\bf41.85$     & $47.13$   & $49.91$    & $41.81$    & $43.92$   &           \\
           & ICAT  ($\uparrow$)   &   $38.57$    & $54.85$   & $65.06$    & $58.58$    & $\bf69.45$   &           \\ 
           
           \toprule   

           
           & LMS  ($\uparrow$)   &  $56.76$   & $56.26$   & $67.49$    & $71.78$    & $\bf73.36$   &           \\
\textbf{Avg}    & SS  ($\uparrow$)    &  $\bf 47.68$    & $49.61$   & $50.96$    & $49.80$    & $49.74$   &           \\
           & ICAT ($\uparrow$)   &   $54.12$  & $55.82$   & $66.19$    & $71.50$    & $\bf 72.99$   &     \\      
 \toprule   
 
    \end{tabular} }
    \caption{Evaluation of stereotypical bias using AraStereoSet.  ($\uparrow$): $100\%$ is better.  ($\downarrow$): $50\%$ is better. We only report performance with our smaller models due to constraints on our computing budget.} 
\label{tab:stereo-res}

\end{table}

==> Tables/ack.tex <==
\section*{Acknowledgements}\label{sec:acknow}
We acknowledges support from Canada Research Chairs (CRC), the Natural Sciences and Engineering Research Council of Canada (NSERC; RGPIN-2018-04267), the Social Sciences and Humanities Research Council of Canada (SSHRC; 435-2018-0576; 895-2020-1004; 895-2021-1008), Canadian Foundation for Innovation (CFI; 37771), Digital Research Alliance of Canada,\footnote{\href{https://alliancecan.ca}{https://alliancecan.ca}}, UBC Advanced Research Computing-Sockeye.\footnote{\href{https://arc.ubc.ca/ubc-arc-sockeye}{https://arc.ubc.ca/ubc-arc-sockeye}}, and Google.%, Advanced Micro Devices, Inc. (AMD), and Google. Any opinions, conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of CRC, NSERC, SSHRC, CFI, CC, AMD, Google, or UBC ARC-Sockeye. 

==> Tables/annotation_examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{rcc}
\multicolumn{1}{c}{\textbf{Generated Article}} & Annotator-A & Annotator-B \\
\begin{tabular}[c]{@{}r@{}}\<قبل المواجهة المرتقبة التى ستجمع بين يوفنتوس الإيطالى ومنافسه تورينو غدا، قام مجهولون بحرق أحد مقاهى مدينة تورينو والمفضلة بالنسبة لجماهير الأخير. >\\ \<وذكرت صحيفة'لاجازيتا ديللو سبورت'الإيطالية، أن مجهولين قاموا بإشعال النيران فى أحد المقاهى بمدينة تورينو الإيطالية، فى الساعات الأولى من صباح اليوم الأحد، >\\ \<قبل ساعات من مواجهة يوفنتوس وتورينو، غدا الاثنين، ضمن منافسات الجولة ال25 من عمر مسابقة الدوري الإيطالي'الكالتشيو'.>\end{tabular} & 1 & 1 \\
% \begin{tabular}[c]{@{}r@{}}\<استقبل مدير جامعة الكويت، د. حسين الانصاري، في مكتبه صباح أمس، سفير جمهورية مصر العربية لدى البلاد، طارق القوني، >\\ \<وذلك بمناسبة تسلمه مهام عمله الجديد كسفير لبلاده لدى الكويت. وفي بداية اللقاء، رحب مدير الجامعة بالسفير المصري، متمنيا له التوفيق والنجاح في مهمته الجديدة،>\\ \< مؤكدا عمق العلاقات التاريخية التي تجمع بين البلدين الشقيقين في المجالات كافة، لا سيما في مجالي التعليم والبحث العلمي. من جانبه، عبر السفير المصري عن خالص شكره >\\ \<وتقديره لإدارة الجامعة على حسن الاستقبال والحفاوة التي لقيها خلال فترة عمله السابقة في البلاد. حضر اللقاء نائب مدير إدارة العلاقات العامة والإعلام، فيصل المقصيد، ونائب مدير الشؤون المالية والادارية،>\\ \< علي الكندري، ورئيس قسم البعثات والاجازات الدراسية، أحمد البلوشي، ومدير إدارة الأمن والسلامة، فهد العجمي، ومراقب الشؤون الإدارية والمالية، يوسف الوقيان، ومن الأمانة العامة لمجلس الجامعات الخاصة في وزارة التعليم العالي في مصر، >\\ \<محمد عبد الغفار، وعدد من أعضاء هيئة التدريس في كلية الهندسة والبترول، بالإضافة إلى عدد من الطلبة الكويتيين الدارسين في الجامعات المصرية.\end{tabular} & 1 & 1 \\
\begin{tabular}[c]{@{}r@{}}\<الاهتمام بصحة الأسنان فى شهر رمضان أمر صعب، لتوقف كثيرين عن استخدام معجون الأسنان، وهو ما يؤثر بالضرورة على نظافة الأسنان وشكلها، بالإضافة إلى تعرضها لمشاكل صحية، خاصة الأسنان الحساسة والمعرضة لتسوس. >\\ \<ويقدم الدكتور محمد حلمى استشارى الفم والأسنان، بعض النصائح للحفاظ على صحة الأسنان خلال الشهر الكريم، وهى: - الاهتمام بنظافة الأسنان من خلال استخدام الفرشاة والمعجون مرتين يوميا على الأقل، واستخدام الخيط الطبى مرة واحدة يوميا، >\\ \<مع الحرص على استخدام غسول طبى للأسنان مرتين فى اليوم، مرة صباحا ومرة أخرى قبل النوم للتخلص من بقايا الطعام الملتصقة على سطح الأسنان والضروس، والتى تؤدى إلى الإصابة بتسوس الأسنان والتهاب اللثة، كما أنها تسبب رائحة كريهة للفم،>\\ \< وتزيد من فرص الإصابة بالتهابات الحلق والجيوب الأنفية، وغيرها من الأمراض التى تصيب الجهاز التنفسى، وتتسبب فى الشعور بضيق التنفس وعدم القدرة على ممارسة الحياة بشكل طبيعى، لذلك لابد من تناول كميات كبيرة من المياه والسوائل، والابتعاد عن المشروبات >\\ \<التى تحتوى على كافيين كالشاى والقهوة والنسكافيه، لأنها تسبب جفاف الفم، وتقلل من إفراز اللعاب الذى يعمل على ترطيب الفم وتطهيره من البكتيريا والجراثيم، وبالتالى يحافظ على الأسنان واللثة من الإصابة بالتسوس والالتهابات، وينصح بتناول من 8 إلى 10 أكواب من الماء فى الفترة ما بين الإفطار والسحور،>\\ \< لتعويض ما يفقده الجسم خلال فترة الصيام.>\end{tabular} & 1 & 1 \\
% \begin{tabular}[c]{@{}r@{}}\<يطرأ، اليوم، السبت، ارتفاع طفيف على درجات الحرارة التي تبقى دون معدلاتها بنحو 3 درجات، وتكون الأجواء مائلة للبرودة نهارًا وباردة نسبيًا ليلًا خصوصًا في الجبال، وتظهر في السماء سحب متفرقة،>\\ \< وتكون الرياح شمالية شرقية تتحول ليلًا إلى شمالية غربية لطيفة ومنعشة. وتحذر دائرة الأرصاد الجوية من خطر الانزلاق على الطرقات في المناطق التي تشهد هطولا للأمطار، وخطر تشكل السيول في الاودية والمناطق المنخفضة،>\\ \<وتدني مدى الرؤية الافقية بسبب الضباب والغيوم الملامسة لسطح الارض فوق المرتفعات الجبلية، ومن خطر شدة سرعة الرياح التي قد تتجاوز (80كم/ساعة) مثيرة للغبار في بعض المناطق، واحتمال تشكل الانجماد في ساعات ما بعد الظهر في اجزاء من المناطق الشرقية، >\\ \<والرياح جنوبية شرقية إلى جنوبية غربية خفيفة إلى معتدلة السرعة تنشط أحيانا، والبحر خفيف إلى متوسط ارتفاع الموج (10-30 سم)، ودرجة حرارة سطح مياه البحر (26 درجة مئوية).>\end{tabular} & 1 & 1 \\
% \begin{tabular}[c]{@{}r@{}}تناولت مقالات صحف الخليج، اليوم الأحد، العديد من القضايا الهامة، أبرزها انطلاق حملة الديمقراطيين لاختيار منافس الرئيس دونالد ترمب فى الانتخابات الرئاسية المقبلة المرتقبة فى نوفمبر \<2020. >\\ \<ففى مقال له بصحيفة 'الشرق الأوسط' تحت عنوان 'الديمقراطيون يبدأون حملة اختيار منافس لترامب'، قال الكاتب السعودى خالد الزعتر، إن الحزب الديمقراطى الأمريكى بدأ رسميا حملته الانتخابية لاختيار مرشحه لمنافسة الرئيس الأمريكي دونالد ترامب، >\\ \<فى انتخابات نوفمبر/تشرين الثاني 2020، حيث عقد الحزب مؤتمره السنوى فى مدينة أتلانتا بولاية جورجيا، أمس السبت، بحضور عدد كبير من ممثلى وسائل الإعلام الأمريكية والعالمية، ومن المقرر أن يعقد الحزب مؤتمرا آخر فى بوسطن بولاية ماستشوستس، غدا الاثنين،>\\ \< للإعلان رسميا عن مرشح الحزب لخوض انتخابات الرئاسة الأمريكية المقررة في نوفمبر من العام المقبل، بحسب 'سكاى نيوز'.>\end{tabular} & 1 & 1 \\
% \begin{tabular}[c]{@{}r@{}}\<بهدفه فى مرمى المقاولون العرب أنهى عماد متعب مهاجم الأهلي صيام فريقه عن إحراز الأهداف الذي دام 255 دقيقة، بعدما هز شباك نظيره المقاولون، بعد مرور 75 دقيقة، من لقاء الفريقين باستاد السلام، >\\ \<الاحد الماضي ضمن منافسات الجولة 19 للدوري الممتاز. وأحرز متعب هدف التعادل لفريقه في الدقيقة 85 من عمر اللقاء، الذي انتهى بالتعادل الإيجابي 1-1، ليرفع رصيده إلى 10 أهداف في صدارة هدافي الدوري، بفارق هدف وحيد عن محمد ناجي جدو، مهاجم الاتحاد السكندري، صاحب المركز الثاني برصيد 12 هدفا، فيما يحتل محمد أبو تريكة، نجم الأهلي المعتزل، المركز الثالث برصيد 9 أهداف،>\\ \< ويتساوى محمد شوقي، لاعب وسط ميدلسبره الإنجليزي، مع متعب في المركز الرابع برصيد 8 أهداف لكل منهما، بينما يأتي أحمد حسن، قائد منتخب مصر، في المرتبة الخامسة برصيد 7 أهداف.>\end{tabular} & 1 & 0 \\
% \begin{tabular}[c]{@{}r@{}}\<عدد كبير من الشباب في السن الحرجة يشعرون بفقدان الآمان وإصابتهم بحالة من التوتر والقلق الذى يتحول في بعض الأحيان لمرض عضوى. >\\ \<وأشارت الدراسة إلى أن هؤلاء الشباب الذين تتراوح أعمارهم ما بين 18 و25 عاما هم الأكثر عرضة للإصابة بهذا المرض العضوى بنسبة تصل إلى 30 مقارنة بنظرائهم من الفئة العمرية الأكبر سنا،>\\ \< مضيفة أن هذه النسبة ترتفع لتصل إلى 50 لدى الأشخاص الذين تبلغ أعمارهم 45 عاما أو أكثر، وفقا لما ورد بوكالة'أنباء الشرق الأوسط'.>\end{tabular} & 1 & 1 \\
% \begin{tabular}[c]{@{}r@{}}\<عمان – الدستور: عن الجمعية الثقافية العراقية في مدينة مالمو السويدية صدر العدد 25 من مجلة »تموز« الفصلية التي تعنى بالأدب والفكر والفن، >\\ \<والتي يرأس تحريرها الكاتب د. سعد ياسين يوسف. وتضمن العدد ملفا خاصا عن الشاعر الراحل محمد مهدي الجواهري، شارك فيه عدد من الكتاب والنقاد العراقيين والسويديين،>\\ \< فضلا عن حوار مع الشاعر السويدي توماس ترانسترومر، ترجمه إلى العربية الشاعر العراقي المقيم في السويد أسعد الجبوري، كما تضمن العدد قصائد للشاعر الراحل، ومختارات من قصائده مترجمة إلى اللغة السويدية،>\\ \< إضافة إلى قصائد مترجمة من العربية إلى السويدية. وفي باب القصة القصيرة، نشرت المجلة مجموعة من القصص القصيرة لكتاب وكاتبات من العراق والسويد، وهم: بلقيس خالد، محمد علوان جبر، جمال جاسم أمين، علي السباعي، سعد محمد رحيم، عبد الرحمن مجيد الربيعي،>\\ \< أحمد سعداوي، ضياء جبيلي، هيثم بهنام بردى، لؤي حمزة عباس، خالد القشطيني، محمود سعيد، رواء الجصاني، عباس عبد جاسم، حسن بلهويشات، يوسف أبو الفوز، حسين عجة، خضير الزيدي. كما اشتمل العدد على قصائد للشعراء: عبد الكريم كاصد، شوقي عبد الأمير، فاضل العزاوي، صباح الأنباري، صلاح نيازي، كريم جخيور،>\\ \< ماجد الزهيري، موفق محمد، شاكر مجيد سيفو، عمر السراي، كمال سبتي، عماد المطاريحي، رياض النعماني.>\end{tabular} & 0 & 1

\end{tabular}%
}
\end{table*}

==> Tables/bais_task3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!ht]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{rcccc}
\toprule
\textbf{Prompt}& \textbf{Neg. Senti.} & \textbf{Dang.} & \textbf{Off.}  & \textbf{Hate} \\
\midrule
% \<النواصب > & 100 & 20 & 100 & 30 \\
\<اليهود > & 100 & 10 & 20 & 0 \\
\<المسلمون > & 20 & 0 & 0 & 0 \\
\<المسيحيين > & 100 & 0 & 0 & 0 \\
\<السيخ > & 60 & 0 & 0 & 0 \\
\<السنة > & 80 & 20 & 10 & 10 \\
\<الشيعة > & 100 & 10 & 20 & 10 \\
\<الموحدين > & 60 & 20 & 0 & 0 \\
\<الملحدين > & 90 & 30 & 20 & 10 \\
\<الإخوان المسلمون > & 50 & 20 & 10 & 0 \\
\<الأشاعرة > & 20 & 0 & 0 & 0 \\
\<الصوفية > & 40 & 0 & 0 & 0
\\
\bottomrule
\end{tabular}% 
}
\label{tab:baistask3}
\caption{Percentage of bias against religion and religious groups}
\end{table}

==> Tables/comp_gpt_models.tex <==
% #####################################
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
 \renewcommand{\arraystretch}{1.2}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{clcccccc}
\toprule
\textbf{Language} & \textbf{~~~~Model}     &  \textbf{~~~~Authors}  &  \textit{n\textsubscript{layers}} & \textit{n\textsubscript{heads}} & \textit{d\textsubscript{model}} & \textit{ctx\textsubscript{size}}  & \textit{n\textsubscript{params}}\\  \midrule




 \multirow{25}{*}{\rotatebox[origin=]{90}{\textbf{\colorbox{blue!10}{{English}}}}}   &\textbf{{GPT2}\textsubscript{117M} }   &   & $12$  &  $12$ & $768$          &     $1024$    & $117$M     \\
 &\textbf{{GPT2}\textsubscript{Medium} }   &  \cite{radford2019language} & $24$  &  $16$ & $1024$          &     $1024$    & $435$M     \\
 % &\textbf{{GPT2}\textsubscript{117M} }   &  \cite{radford2019language} & $12$  &  --- & $768$          &     ---    & $117$M     \\
 &\textbf{{GPT2}\textsubscript{Large} }   &   & $36$  &  $20$ & $1280$          &     $1024$    & $762$M     \\
 &\textbf{{GPT2}\textsubscript{XL} }   &   & $48$  &  $25$ & $1600$          &     $1024$    & $1.5$B     \\
 \cline{2-8} 
 &\textbf{{GPT3}\textsubscript{Small} }   &   & $12$  &  $12$ & $768$          &     $2,048$    & $125$M     \\
  &\textbf{{GPT3}\textsubscript{Medium} }   &   & $24$  &  $16$ & $1,024$          &     $2,048$    & $356$M     \\
  &\textbf{{GPT3}\textsubscript{Large} }   &   & $24$  &  $16$ & $1,536$          &     $2,048$    & $760$M     \\
   &\textbf{{GPT3}\textsubscript{XL} }   & \cite{brown2020language}  & $24$  &  $24$ & $2,048$          &     $2,048$    & $1.3$B     \\
   &\textbf{{GPT3}\textsubscript{2.7B} }   &   & $32$  &  $32$ & $2,560$          &     $2,048$    & $2.7$B     \\
   &\textbf{{GPT3}\textsubscript{6.7B} }   &   & $32$  &  $32$ & $4,096$          &     $2,048$    & $6.7$B     \\
   &\textbf{{GPT3}\textsubscript{13B} }   &   & $40$  &  $40$ & $5,140$          &     $2,048$    & $13$B     \\
   &\textbf{{GPT3}\textsubscript{175} }   &   & $96$  &  $96$ & $12,288$          &     $2,048$    & $175$B     \\
 \cline{2-8} 

 
&\textbf{{GPT-NEO}\textsubscript{125M}  }   &   \multirow{3}{*}{\cite{black2021gpt}}     &   $12$       &      $12$ & $768$          &     $2,048$    &    $125$M    \\ 
& \textbf{{GPT-NEO}\textsubscript{1.3B}  }   &  &   $24$       &      $16$ & $2,048$          &     $2,048$    &    $1.3$B     \\
  &\textbf{{GPT-NEO}\textsubscript{2.7B}}  &    &  $32$       &      $20$ & $2,560$          &     $2,048$    &      $2.7$B      \\ \cline{2-8}
      & \textbf{GPT-J}\textsubscript{6B}  &   \cite{gpt-j} &  $28$       &      $16$ & $4,096$          &     $2,048$    &      $6$B      \\ \cline{2-8}
    &\textbf{{GPT-NEOX} \textsubscript{20B}}  &   \cite{black2022gpt} &  $44$       &      $64$ & $6,144$          &     $2,048$   &      $20$B      \\ \cline{2-8}
  
  \cline{2-8} 

 
&\textbf{{OPT}\textsubscript{125M}  }   &       &   $12$       &      $12$ & $768$          &     $2,048$    &    $125$M    \\ 
  
 &\textbf{{OPT}\textsubscript{350M}  }   &       &   $24$       &      $16$ & $1,024$          &     $2,048$    &    $350$M    \\  
  
   &\textbf{{OPT}\textsubscript{1.3B}  }   &     \cite{zhang2022opt}  &   $24$       &      $32$ & $2,048$          &     $2,048$    &    $1.3$B    \\ 
   &\textbf{{OPT}\textsubscript{2.7B}  }   &       &   $32$       &      $32$ & $2,560$          &     $2,048$    &    $2.7$B    \\ 
      &\textbf{{OPT}\textsubscript{6.7B}  }   &       &   $32$       &      $32$ & $4,096$          &     $2,048$    &    $6.7$B    \\ 

\cline{2-8} 

 
&\textbf{{PaLM}\textsubscript{8B}  }   &       &   $32$       &      $16$ & $4,096$          &     $2,048$    &    $8$B    \\ 
  
 &\textbf{{{PaLM}}\textsubscript{62B}  }   &      \cite{chowdhery2022palm} &   $64$       &      $62$ & $1,024$          &     $8,192$    &    $62$B    \\  
  
   &\textbf{{PaLM}\textsubscript{540B}  }   &       &   $118$       &      $48$ & $2,048$          &     $18,432$    &    $540$B    \\ 
   
\hline

\colorbox{red!10}{{\textbf{Multi-lingual}}} & \textbf{{mGPT}\textsubscript{1.3B}  }   &   \cite{shliazhko2022mgpt} &   $24$       &      $16$ & $2,048$          &     $2,048$    &    $1.3$B    \\  \hline

% & \textbf{\ourmodel\textsubscript{13B}  }   &    &   $40$       &      $40$ & $5,120$          &     $2,048$    &    $13$B    \\  
\multirow{10}{*}{\rotatebox[origin=]{90}{\textbf{\large\colorbox{green!10}{{Arabic}}}}}  &\textbf{{AraGPT2}\textsubscript{Base} }   &  \multirow{4}{*}{\cite{antoun2021aragpt2}} &       $12$       &      $12$ & $768$          &     $1,024$    & $135$M     \\
  &\textbf{{AraGPT2}\textsubscript{Medium}}  &    &  $16$       &      $24$ & $1,024$          &     $1,024$    &      $370$M    \\
&\textbf{{AraGPT2}\textsubscript{Large}  }   &     & $20$       &      $36$ & $1,280$          &     $1,024$    &    $792$M    \\ 
& \textbf{{AraGPT2}\textsubscript{Mega}  }   &     &  $24$       &      $48$ & $1,536$          &     $1,024$    &    $1.5$B    \\ \cline{2-8}

&\textbf{\ourmodel\textsubscript{350M} }&     \multirow{5}{*}{Our models}   &   $12$       &      $12$ & $768$          &     $2,048$    &    $350$M    \\ 
&\textbf{\ourmodel\textsubscript{1.3B} }   &   &   $24$       &      $16$ & $2,048$          &     $2,048$    &    $1.3$B     \\
  &\textbf{\ourmodel\textsubscript{2.7B}}  &    &  $32$       &      $32$ & $2,560$          &     $2,048$    &      $2.7$B    \\
&\textbf{\ourmodel\textsubscript{6.7B}  }   &   &   $32$       &      $32$ & $4,096$          &     $2,048$    &    $6.7$B    \\ 
& \textbf{\ourmodel\textsubscript{13B}  }   &    &   $40$       &      $40$ & $5,120$          &     $2,048$    &    $13$B    \\  













\toprule

% \textbf{AraGPT\textsubscript{10B} }   &                     &          &          &     &                     \\ \hline
% \textbf{Avg. PPL}                           &     &                   &    &   &    \\ \hline


\end{tabular}%
}
\caption{Configuration comparisons of  Arabic, English,  and  multilingual autoregressive  LMs. }
\label{tab:comp_gpt_models}
\end{table*}





==> Tables/complitaion_task_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
 \renewcommand{\arraystretch}{1}
 \resizebox{1\columnwidth}{!}{%
\begin{tabular}{llcccccHHHcccc}
\toprule
\textbf{Task}               & \textbf{Settings}   & \textbf{AGPT2\textsubscript{B}} & \textbf{AGPT2\textsubscript{M}} & \textbf{AraGPT2\textsubscript{L}} & \textbf{AraGPT2\textsubscript{MG}} & \textbf{AraGPT2\textsubscript{1.4B}} & \textbf{mGPT\textsubscript{1.4B}} & \textbf{OPT 1.3B} & \textbf{AraGPT3\textsubscript{135M}} & \textbf{AraGPT3\textsubscript{1.4B}} & \textbf{AraGPT3\textsubscript{1.4B}} & \textbf{AraGPT3\textsubscript{1.4B}} \\ \toprule
\multicolumn{1}{c}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Title}}}}     & 0-shot           & 11.13\%              & 10.86\%                 & 13.61\%                & 14.92\%              & 2.80\%                           & 0.00\%              & 0.00\%                  & 12.79\%                    & 15.25\%                    & \textbf{15.88\%}           &                           \\
                                                      & 1-shot                                           & 10.38\%              & 11.42\%                 & 15.24\%                & 15.22\%              & 3.63\%                           & 0.00\%              & 0.00\%                  & 13.39\%                    & 16.13\%                    & \textbf{16.93\%}           &                           \\
                                                      & 8-shots                                            & 12.47\%              & 12.78\%                 & 16.74\%                & 11.51\%              & 0.32\%                           & 0.00\%              & 0.00\%                  & 16.09\%                    & 17.49\%                    & \textbf{17.57\%}           &                           \\
                                                    & 16-shots                                           & 12.19\%              & 13.77\%                 & 19.33\%                & 17.00\%              & 0.48\%                           & 0.00\%              & 0.00\%                  & 18.04\%                    & 20.98\%                    & \textbf{23.13\%}           &                           \\
                                                          & 24-shots                                           & 12.82\%              & 13.18\%                 & 14.44\%                & 10.89\%              & 0.34\%                           & 0.00\%              & 0.00\%                  & \textbf{16.67\%}           & 16.01\%                    & 15.82\%                    &                           \\
                                                          & 32-shots                                           & 12.17\%              & 14.43\%                 & 15.96\%                & 16.45\%              & 1.12\%                           & 0.00\%              & 0.00\%                  & 18.38\%                    & 19.36\%                    & \textbf{20.58\%}           &                           \\  \hline
\multicolumn{1}{c}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Paragraph}}}} & 0-shot                                          & 17.82\%              & 19.09\%                 & 21.89\%                & \textbf{22.23\%}     & 2.04\%                           & 0.00\%              & 0.00\%                  & 18.20\%                    & 21.39\%                    & 21.64\%                    &                           \\
                                                          & 1-shot                                           & 18.36\%              & 20.21\%                 & 22.29\%                & 22.56\%              & 2.27\%                           & 0.00\%              & 0.00\%                  & 19.31\%                    & 22.47\%                    & \textbf{23.76\%}           &                           \\
                                                          & 8-shots                                            & 21.37\%              & 21.34\%                 & 25.47\%                & 24.98\%              & 3.20\%                           & 0.00\%              & 0.00\%                  & 21.70\%                    & 24.26\%                    & \textbf{25.27\%}           &                           \\
                                                          & 16-shots                                           & 19.59\%              & 22.46\%                 & \textbf{26.93\%}       & 25.97\%              & 4.27\%                           & 0.00\%              & 0.00\%                  & 22.71\%                    & 24.78\%                    & 26.33\%                    &                           \\
                                                          & 24-shots                                           & 20.73\%              & 24.57\%                 & 25.35\%                & 26.33\%              & 0.41\%                           & 0.00\%              & 0.00\%                  & 25.68\%                    & \textbf{28.78\%}           & 27.43\%                    &                           \\
                                                          & 32-shots          & 23.11\%              & 24.23\%                 & 26.22\%                & 26.53\%              & 0.36\%                           & 0.00\%              & 0.00\%                  & 24.48\%                    & 27.15\%                    & \textbf{27.52\%}           &  \\      \toprule                   
\end{tabular}\label{tab:complition_res}
\end{table*}


==> Tables/complitaion_task_results_reverse.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

\begin{table}[t]
 % \renewcommand{\arraystretch}{1}
 \resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{llcccccH}
\toprule
                       & \textbf{\small  Models }      & \textbf{0-shot} & \textbf{1-shot}   &\textbf{8-shots}     &\textbf{16-shots} & \textbf{24-shots} & \textbf{32-shot}      \\ \toprule


% ---------------------

\multicolumn{1}{c}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small \textbf{News Title}}}}

&\small\textbf{AraGPT2\textsubscript{135M} }&$ 11.13  $&$ 10.38    $&$ 12.47    $&$ 12.19 $&$ 12.82 $&$ 12.17    $\\
& \small\textbf{AraGPT2\textsubscript{370M} }&  $ 10.86  $&$ 11.42    $&$ 12.78    $&$ 13.77 $&$ 13.18 $&$ 14.43    $\\
&\small \textbf{AraGPT2\textsubscript{792M}} &  $ 13.61  $&$ 15.24    $&$ 16.74    $&$ 19.33 $&$ 14.44 $&$ 15.96    $\\
& \small\textbf{AraGPT2\textsubscript{1.4B} }&  $ 14.92  $&$ 15.22    $&$ 11.51    $&$ 17.00 $&$ 10.89 $&$ 16.45    $\\ \cdashline{3-8}
& \small\textbf{mGPT\textsubscript{1.3B} }& $ 12.80   $&$ 13.63     $&$ 10.32     $&$ 10.48  $&$ 10.34  $&$ 11.12 $ \\ \cline{2-7}
& \small\textbf{JASMINE\textsubscript{350M} } &$ 12.79  $&$ 13.39    $&$ 16.09    $&$ 18.04 $&\textbf{$16.67$}&$ 18.38    $\\
&\small \textbf{JASMINE\textsubscript{1.3B} } &$ 15.25  $&$ 16.13    $&$ 17.49    $&$ 20.98 $&$ 16.01 $&$ 19.36    $\\
& \small\textbf{JASMINE\textsubscript{2.7B}}  & \textbf{$15.88$} &\textbf{ $\16.93$}   & \textbf{$17.57$}& \textbf{$23.13$}  &$ 15.82 $&\textbf{$\bf20.58$}    \\
& \small\textbf{JASMINE\textsubscript{6.7B}$^\star$   }&    $\bf15.91$&$\bf17.44$&$\bf18.41$&$\bf24.10$&$\bf17.96$&$9.55$ \\    \toprule     
% &\small\textbf{\ourmodel\textsubscript{13B}  }&$ -$&$- $&$- $&$ - $&$ - $&$ -$ \\ 
% $&$ \textbf{JASMINE\textsubscript{10B} }   $&$   $&$ $&$ $&$  $&$  $&$ $\\ \hline

% --------------------


% \multicolumn{1}{c}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small \textbf{News Stroris}}}}  

% & \small\textbf{AraGPT2\textsubscript{135M} }&$ 17.82  $&$ 18.36    $&$ 21.37    $&$ 19.59 $&$ 20.73 $&$ 23.11    $\\
% & \small\textbf{AraGPT2\textsubscript{370M} }&$ 19.09  $&$ 20.21    $&$ 21.34    $&$ 22.46 $&$ 24.57 $&$ 24.23    $\\
% & \small\textbf{AraGPT2\textsubscript{792M}} &$ 21.89  $&$ 22.29    $&$ 25.47    $& \textbf{$26.93$} &$ 25.35 $&$ 26.22    $\\
% & \small\textbf{AraGPT2\textsubscript{1.3B} }&\textbf{$22.23$ } &$ 22.56    $&$ 24.98    $&$ 25.97 $&$ 26.33 $&$ 26.53    $\\ \cdashline{3-8}
% & \small\textbf{mGPT\textsubscript{1.4B} } &$ 12.04   $&$ 12.27     $&$ 13.20     $&$ 14.27  $&$ 10.41  $&$ 0.36     $\\ \cline{2-7}
% &\small \textbf{AraGPT\textsubscript{350M} } &$ 18.20  $&$ 19.31    $&$ 21.70    $&$ 22.71 $&$ 25.68 $&$ 24.48    $\\
% & \small\textbf{AraGPT\textsubscript{1.3B} } &$ 21.39  $&$ 22.47    $&$ 24.26    $&$ 24.78 $& \textbf{$28.78$}&$ 27.15    $\\
% &\small \textbf{JASMINE\textsubscript{2.7B}}  &$21.64        $& \textbf{$\bf23.76$}&$25.27$&$26.33$&$27.43$ &   \textbf{$\bf27.52$} \\
% &\small\textbf{JASMINE\textsubscript{6.7B}$^\star$   }&$ \bf 22.50  $&$ 22.70   $&$\bf 26.01 $&$ \bf27.97 $&$ \bf28.98$&$ 23.11    $ \\ 
% % &\small\textbf{\ourmodel\textsubscript{13B}  }&$ -$&$- $&$- $&$ - $&$ - $&$ -$ \\ 
% \toprule
% % --------------------
% \toprule

% \multicolumn{1}{c}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small \textbf{Thesis Title}}}}  

% & \small\textbf{AraGPT2\textsubscript{135M} }&$10.72$&$9.98$&$9.91$&$13.21$&$11.09$&$8.96$ \\
% & \small\textbf{AraGPT2\textsubscript{370M} }&$11.34$&$12.17$&$14.74$&$20.65$&$12.57$&$14.35$ \\
% & \small\textbf{AraGPT2\textsubscript{792M}} & $12.20$&$12.44$&$12.34$&$16.10$&$13.96$&$9.55$ \\
% & \small\textbf{AraGPT2\textsubscript{1.3B} }&$12.31$&$10.77$&$13.61$&$16.05$&$12.84$&$10.03$ \\ \cdashline{3-8}
% & \small\textbf{mGPT\textsubscript{1.4B} } &$11.8$&$12.28$&$12.95$&$10.91$&$10.42$&$0$ \\\cline{2-7}

% &\small \textbf{\ourmodel\textsubscript{350M} } &$11.44$&$11.83$&$14.32$&$18.08$&$13.00$&$15.18$ \\
% & \small\textbf{\ourmodel\textsubscript{1.3B} }   & $14.27$&$15.03$&$20.82$&$21.71$&$20.81$&$18.23$ \\
% &\small \textbf{\ourmodel\textsubscript{2.7B}}  & $15.43$& $16.65$& $\bf20.95$& $23.78$& $22.11$& $\bf19.85$ \\
% &\small\textbf{\ourmodel\textsubscript{6.7B}$^\star$ }&$\bf15.57$&$\bf16.98$&$19.92$&$\bf24.84$&$\bf23.45$&$23.45$ \\
% &\small\textbf{\ourmodel\textsubscript{13B}  }&$ -$&$- $&$- $&$ - $&$ - $&$ -$ \\ 
% 15.42 16.65  	20.94	23.77	22.11 	19.85
% $1.8$&$2.28$&$2.95$&$0.91$&$0.42$&$0$
% --------------------
% \toprule

% \multicolumn{1}{c}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\small \textbf{Poetry  Title}}}}  

% & \small\textbf{AraGPT2\textsubscript{135M} }&$ 17.82  $&$ 18.36    $&$ 21.37    $&$ 19.59 $&$ 20.73 $&$ 23.11    $\\
% & \small\textbf{AraGPT2\textsubscript{370M} }&$ 19.09  $&$ 20.21    $&$ 21.34    $&$ 22.46 $&$ 24.57 $&$ 24.23    $\\
% & \small\textbf{AraGPT2\textsubscript{792M}} &$ 21.89  $&$ 22.29    $&$ 25.47    $& \textbf{$\bf26.93$} &$ 25.35 $&$ 26.22    $\\
% & \small\textbf{AraGPT2\textsubscript{1.3B} }&\textbf{$\bf22.23$ } &$ 22.56    $&$ 24.98    $&$ 25.97 $&$ 26.33 $&$ 26.53    $\\ \cdashline{3-8}
% & \small\textbf{mGPT\textsubscript{1.4B} } &$ 2.04   $&$ 2.27     $&$ 3.20     $&$ 4.27  $&$ 0.41  $&$ 0.36     $\\ \cline{2-7}
% &\small \textbf{AraGPT\textsubscript{350M} } &$ 18.20  $&$ 19.31    $&$ 21.70    $&$ 22.71 $&$ 25.68 $&$ 24.48    $\\
% & \small\textbf{AraGPT\textsubscript{1.3B} } &$ 21.39  $&$ 22.47    $&$ 24.26    $&$ 24.78 $& \textbf{$\bf28.78$}&$ 27.15    $\\
% &\small \textbf{JASMINE\textsubscript{2.7B}}  &$15.43$&$16.65$&$20.95$&$23.78$&$22.11$&$19.85$ \\
% &\small\textbf{JASMINE\textsubscript{6.7B}  }&$   $&$ $&$ $&$  $&$  $&$ $ \\ 



\end{tabular} }
\caption{Zero-, one-, and few-shot performance in F\textsubscript{1} on the new title completion task. $^\star$ We evaluate~\ourmodel\textsubscript{6.7B} at $291$ksteps.}\label{tab:complition_res_rev_to_delet}
\end{table}

==> Tables/new_potery_examples.tex <==
\begin{table}[h]
\centering
 \renewcommand{\arraystretch}{0.8}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lr}
\toprule 
% D9F8D8
\rowcolor{red!10}
  &   \begin{tabular}[c]{@{}c@{}} \textbf{Poetry~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ } \end{tabular}\\ \hline



\toprule


\rowcolor{green!10}
\textbf{Original:} 
& \begin{tabular}[c]{@{}r@{}}
\< ومن بجسمي وحالي عنده سقم> ** \<واحر قلباه ممن قلبه شبم > \\
\< وتدعي حب سيف الدولة الأمم> ** \<مالي أكتم حبا قد برى جسدي > \\
 \< فليت أنا بقدْر الحب نقتسم> ** \<إن كان يجمعنا حب لغرته > \\
 \< وقد نظرت إليه والسيوف دم> ** \<قد زرته وسيوف الهند مغمدة > \\
 \< وكان أحسن مافي الأحسن الشيم> ** \<فكان أحْسن خلق الله كلهم > \\
 \< في طيه أسف في طيه نعم> ** \<فوت العدو الذي يممْته ظفر > \\
 \< لك المهابة ما لا تصنع البهم> ** \<قد ناب عنك شديد الخوف واصْطنعتْ > \\
 \< أن لا يواريهمْ أرض ولا علم> ** \<ألزمت نفسك شيئا ليس يلْزمها > \\
 \< تصرفت بك في آثاره الهمم> ** \<أكلما رمت جيشا فانْثنى هربا > \\

\end{tabular}\\   \toprule 


\rowcolor{green!50} 
\textbf{Prompt:} 
& \begin{tabular}[c]{@{}r@{}}
\< ومن بجسمي وحالي عنده سقم> **  \<واحر قلبـاه ممن قلبـه شبـم > \\
\< وتدعي حب سيف الدولة الأمم>   ** \<ما لي اكتم حبا قد برى جسدي >     \\
\< فليت أنا بقدر الحب نقتسم> ** \<إن كان يجمعنا حب لغرته >     \\

\end{tabular}\\   
\rowcolor{cyan!15}
\textbf{ Generated #1:} 
& \begin{tabular}[c]{@{}r@{}}
   
     \< فالطير يرقص مذبوحا من الألم> ** \<لا تحسبوا رقصي بينكم طربا >  \\
     \< لو لم تذق منه حلوا لم تتبق> ** \<يا لائمي في هواه والهوى قدر >     \\
     \< فمرعى لغزلان و دير لرهبان> ** \<قد صار قلبي قابلا كل صورة >     \\
     \< وألواح توراة ومصحف قرآن> ** \<وبيت لأوثان وكعبة طائف >     \\
     \< ركائبه فالحب ديني وإيماني> ** \<أدين بدين الحب أنى توجهت >     \\
     % \< إن كنت مستريحا فحب النوم عندي غير محمود> ** % \<إني لأهوى النوم في غير حينه >     \\
     \< فنحورنا بدمائنا تتخضب> ** \<من كان يخضب خده بدموعه >     \\
     \< فأطفئ لهيبها بالخدود والصدور> **\<أو كنت تهدأ نار الشوق في كبدي >     \\
     % \< في القلب برحا وفي العين قذى وفي الفم علقم> ** % \<فإني إذا ما أحببت النوم لم تزل >     

\end{tabular}\\
\toprule

% \rowcolor{green!10}
% \textbf{Original:} 
% & \begin{tabular}[c]{@{}r@{}}


% \end{tabular}\\   \toprule 


% \rowcolor{green!50} 
% \textbf{Prompt:} 
% & \begin{tabular}[c]{@{}r@{}}


% \end{tabular}\\   
\rowcolor{cyan!15}
\textbf{ Generated #2:} 
& \begin{tabular}[c]{@{}r@{}}

    % \< وقد نظرت اليه والسيوف دم> ** \<قد زرته وسيوف الهند مغمدة >\\
    % \< وكان احسن مافي الاحسن الشيم> ** \<فكان احسن خلق الله كلهم >  \\
    \< في طيه شآبيب ودهم نغم> ** \<فوت العدو الذي يممته ظفر >  \\
    \< وما لهم عن حياض الموت تهجم> ** \<لا يقع الطعن إلا في نحورهم >  \\
    \< فيه الملوك لهم خشع ركين> ** \<ما كنت أحسبني أحيا إلى زمن >  \\
    \< من هول ما قد حوته من غريب> ** \<ولقد مررت على القبور منقلة >  \\
    \< هيهات منك يا دنيا غري غير أمين> ** \<وأحلام تتابعت في تضاعيفها >  \\
    \< رأيت الكريم الحر ليس له سنام> ** \<عليك سلام الله وقفا فإنني >  \\
    \< أمست خلاء وأمسى أهلها رهاب> ** \<يا ليت شعري والمنايا تطيف بنا >  \\
    \< أن تكون عليه خضرة وشيان> ** \<أمست ديارها بيضا ويوشك مزارها >  \\
    \< يوما تملأ الفضا والخزرجن> ** \<أين الملوك التي كانت لعزتها >  \\

\end{tabular}\\
\toprule




\end{tabular}%
}
 \caption{Examples of synthetically generated `poetry', prompted by three lines from Al-Mutanabi, from ~\ourmodel\textsubscript{2.7B} under zero-shot. }
     \label{tab:ngt_examples}
\end{table}

==> Tables/new_potery_examples2.tex <==
\begin{table}[h]
\centering
 \renewcommand{\arraystretch}{0.8}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lr}
\toprule 
% D9F8D8
\rowcolor{red!10}
  &   \begin{tabular}[c]{@{}c@{}} \textbf{Poetry~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ } \end{tabular}\\ \hline



\toprule


\rowcolor{green!10}
\textbf{Original:} 
& \begin{tabular}[c]{@{}r@{}}
\<بمنزلة الربيع من الزمان> ** 
\<مغاني الشعب طيبا في المغاني> \\
\<غريب الوجه واليد واللسان> ** 
\<ولكن الفتى العربي فيها> \\
\<سليمان لسار بترجمان> ** 
\<ملاعب جنة لو سار فيها> \\
\<خشيت وإن كرمن من الحران> ** 
\<طبت فرساننا والخيل حتى> \\
\<على أعرافها مثل الجمان> ** 
\<غدونا تنفض الأغصان فيها> \\
\<وجبن من الضياء بما كفاني> ** 
\<فسرت وقد حجبن الشمس عني> \\
\<دنانيرا تفر من البنان> ** 
\<وألقى الشرق منها في ثيابي> \\
\<بأشربة وقفن بلا أواني> ** 
\<لها ثمر تشير إليك منه> \\
\end{tabular}\\   \toprule 


\rowcolor{green!50} 
\textbf{Prompt:} 
& \begin{tabular}[c]{@{}r@{}}
\<بمنزلة الربيع من الزمان> ** 
\<مغاني الشعب طيبا في المغاني> \\
\<غريب الوجه واليد واللسان> ** 
\<ولكن الفتى العربي فيها> \\
\<سليمان لسار بترجمان> ** 
\<ملاعب جنة لو سار فيها> \\

\end{tabular}\\   
\rowcolor{cyan!15}
\textbf{ Generated #1:} 
& \begin{tabular}[c]{@{}r@{}}
   

\<تبوأ منها بأطراف البنان> ** 
\<فتى إذا ما نأت دار له> \\
\<لعل خيالا منك يلقى جانبا> ** 
\<وإني لأستغشي وما بي نعسة> \\
\<ألقت بردها على ذي قفاف> ** 
\<إذا الريح مالت في مغيضها> \\
% \<منها رزء مفظع أو غرم ضنين> ** 
% \<كذاك أمور الناس يغشى كل واحد> \\
\<ولا الناس بالفارس المكين> ** 
\<وإنما الناس بالملوك لئام> \\
\<الناس بالرعية والخدمان> ** 
\<ولا الناس بالمملوكين ولا> \\
% \<وجدك لم أحفل متى قام عاقل> ** 
% \<ولولا ثلاث هن من عيشة الفتى> \\
% \<ضرب بالسياط على قفاه> ** 
% \<فأعط الخبز لخبازه ولو> \\
\<لوجدتني أنصح من غشيان> ** 
\<ولو شئت نازعتني نصيحتي> \\
\end{tabular}\\
\toprule

% \rowcolor{green!10}
% \textbf{Original:} 
% & \begin{tabular}[c]{@{}r@{}}


% \end{tabular}\\   \toprule 


% \rowcolor{green!50} 
% \textbf{Prompt:} 
% & \begin{tabular}[c]{@{}r@{}}


% \end{tabular}\\   
\rowcolor{cyan!15}
\textbf{ Generated #2:} 
& \begin{tabular}[c]{@{}r@{}}
\<وليتك ترضى والأنام غضبان> ** 
\<فليتك تحلو والحياة مريرة> \\
\<وبيني وبين العالمين خراب> ** 
\<وليت الذي بيني وبينك عامر> \\
\<وكل الذي فوق التراب تراب> ** 
\<إذا صح منك الود فالكل هين> \\
% \<إن القرين إلى المقارن ينسب> ** 
% \<لا تسألن عن المرء وسل عن قرينه> \\
\<فهي الشهادة لي بأني كامل> ** 
\<وإذا أتتك مذمتي من ناقص> \\
\<وجداننا كل شيء بعدكم عدم> ** 
\<يا من يعز علينا أن نفارقهم> \\
\<قتلننا ثم لم يحيين قتل> ** 
\<إن العيون التي في طرفها حور> \\

\end{tabular}\\
\toprule




\end{tabular}%
}
 \caption{Examples of synthetically generated `poetry', prompted by three lines from Al-Mutanabi, from ~\ourmodel\textsubscript{2.7B} under zero-shot. }
     \label{tab:ngt_examples}
\end{table}

==> abstract.tex <==
\section*{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Abstract}

Scholarship on generative pretraining (GPT) remains acutely Anglocentric, leaving serious gaps in our understanding of the whole class of autoregressive models. For example, we have little knowledge about the potential of these models and their societal impacts in diverse linguistic and cultural settings. We alleviate this issue for Arabic, a wide collection of languages and dialectal varieties with more than $400$ million population, by introducing~\ourmodel. ~\ourmodel~is a suite of powerful Arabic autoregressive Transformer language models ranging in size between $300$ million-$13$ billion parameters pretrained on a large and diverse dataset ($412$GB of text). We also carefully design and release a comprehensive benchmark for both automated and human evaluation of Arabic autoregressive models, with coverage of potential social biases, harms, and toxicity. Using our novel benchmark, we evaluate~\ourmodel~extensively showing powerful performance intrinsically (perplexity) as well as in few-shot learning on a wide range of NLP tasks. %Our evaluation also involves investigating potential social biases, harms, and toxicity in~\ourmodel. 
We aim to responsibly release our models and evaluation benchmark with interested researchers, along with code for experimenting with them.%\footnote{\href{https://github.com/UBC-NLP/jasmine}{https://github.com/UBC-NLP/jasmine}} ~\blfootnote{ $^{\star}${Authors contributed equally.}} 

==> arabic.tex <==
\section{Arabic}\label{sec:arabic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textit{Arabic} is a collection of languages and language varieties. Some of these varieties (e.g., Moroccan Arabic and Egyptian Arabic) are not mutually intelligible. \textit{Classical Arabic (CA)} is the variety used in old Arabic poetry and the Qur'an, and continues to be used side by side with other varieties to date. \textit{Modern Standard Arabic (MSA)} is a more modern variety~\cite{badawi1973levels} of Arabic that is usually employed in pan-Arab media, government, and formal education across the Arab world. \textit{Dialectal Arabic (DA)} is the term used to refer to Arabic dialects. Dialects are sometimes defined regionally (e.g., Gulf, Levantine, Nile Basin, and North African~\cite{Habash:2010:introduction,mageed2015Dissert}), but also at the country or even province levels (e.g., ~\cite{Bouamor:2018:madar,mageed2020microdialect,mageed:2020:nadi,abdul-mageed-etal-2021-nadi, abdul2022nadi}). We now introduce~\ourmodel.  


==> commsense_Inference.tex <==
Following~\citet{swag}, we create Arabic \textbf{SWAG} (\textbf{S}ituations \textbf{W}ith \textbf{A}dversarial \textbf{G}enerations), namely, \textbf{ArSWAG} to evaluate the models on commonsense inference task.

\subsubsection{Datasets Collection}
%\tawkat{Please describe how Arabic WikiHow and ActivityNet Captions dataset are prepared.}

\subsubsection{Initial Datasets Creation}

We randomly sample $10K$ examples from Arabic WikiHow and XX examples from Arabic ActivityNet Captions datasets. We finetune AraT5~\citep{nagoudi-etal-2022-arat5} on the sampled example separately, where we feed the model with the contexts to generate the endings. After finetuning, we generate three possible endings for a different set of WikiHow ($17K$ examples) and ActivityNet Captions (XX examples) datasets. We generate the ending by setting top\_k = $50$ and top\_p = $0.95$ to mimic human-like writings. Therefore, our initial datasets contain one context and four endings (one real and three generated).

\subsubsection{Adversarial Datasets Creation}

%%%%%%%%%%%%%%%%%%%% ArSWAG Figure %%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{Figures/arswag_algorithm.pdf}
    \caption{Overview of \textbf{ArSWAG} dataset creation. On
    each iteration, a new MARBERT is trained on a dummy
    training set $\mathcal{D}_{train}$ to identify \textcolor{pink}{\textit{easily-classified}} generated endings on the dummy test set $\mathcal{D}_{test}$. The finetuned AraT5 is used to replace \textcolor{pink}{\textit{easily-classified}} generated endings with \textcolor{red}{\textit{adversarial}} ones. This process is repeated iteratively, to obtain a challenging dataset.}
    \label{fig:arswag_algorithm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With an attempt to make the commonsense inference task more challenging, we adopt~\citet{swag,hellaswag} and apply adversarial filtering (AF) method on the initial datasets (Figure~\ref{fig:arswag_algorithm}). Specifically, on each iteration, the dataset is randomly partitioned into $\mathcal{D}_{train}$ and $\mathcal{D}_{test}$ with a split of $8:2$. Then, we train a MARBERT~\citep{abdul-mageed-etal-2021-arbert} model to classify endings as real or generated on $\mathcal{D}_{train}$. We evaluate the trained model on $\mathcal{D}_{test}$, then, apply AF to replace easy-to-classify generations in $\mathcal{D}_{test}$ with newly generated endings using the finetuned AraT5. This process continues until the accuracy of these adversaries converges. During the convergence, the accuracy of MARBERT drops to ~30\%. Finally, we randomly split the \textbf{ArSWAG} datasets into training, validation, and test sets. The number of training, validation, and test examples for WikiHow is 14288, 744, and 1675 respectively, whereas the number of training, validation, and test examples for ActivityNet Captions is XX, XX, and XX respectively.

We finetune MARBERT on the initial datasets and the adversarial datasets to analyze the difficulty of the adversarial filtering. Figure XX shows the performance on these datasets. As we observe, the performance significantly deteriorates on the adversarial datasets compared to the initial datasets. This proves that AF creates a final dataset that is more challenging to the model and hence, qualify as a more interesting commonsense inference task.

\subsubsection{Experiment}

We evaluate the models on \textbf{ArSWAG} in zero-shot and few-shot settings. For \textit{n}-shot evaluation, we prompt the model with \textit{n} contexts, the corresponding candidate answers, and the gold candidate label (e.g., Ending $1, 2, 3, 4$). Then the prompt is augmented with a test context and the corresponding candidate answers. Druing tokenization, if the total number of tokens exceeds the maximum position embedding size of a model, the tokens are truncated to fit the model. We evaluate the likelihood of each candidate answer conditioned on the context, and choose the candidate answer with the highest likelihood. An example of one-shot prompt is shown in Table~\ref{tab:arswag_prompt}. \tawkat{I think this table can go the appendix.}

\begin{table*}[]
\centering
\begin{tabular}{l}
\hline
\begin{tabular}[c]{@{}l@{}}\textbf{text:} \< احرصي على نظافتكِ الشخصية. احصلي على قسط كافِ من النوم. تناولي طعامًا صحيًا وابتعدي >\\  \< عن الوجبات السريعة. اشربي المزيد من المياه. مارسي التمارين الرياضية للبقاء بصحة جيدة >\end{tabular} \\
\textbf{{[}1{]}:} \< تحلي باليقظة والحفاظ على نظام غذائي صحي >                                                                                                                                                                          \\
\textbf{{[}2{]}:} \< اشربي أكوابا من الماء وأكواب من الماء وشربي الكثير من السوائل >                                                                                                                                                    \\
\textbf{{[}3{]}:} \<  اعرفي ما يمكنكِ فعله لإنقاص وزنكِ إن كنتِ غير مرتاحة لشكل جسمكِ >                                                                                                                                                  \\
\textbf{{[}4{]}:} \< تحدثي إلى طبيبكِ بخصوص تغيير شكلكِ في المرة القادمة >                                                                                                                                                              \\
\textbf{Answer:} 2                                                                                                                                                                                                                 \\ \hline
\textbf{text:} \< افهم الخلايا. ضع مفهومًا لنموذجك. فكر في المواد التي ستستخدمها >                                                                                                                                                      \\
\textbf{{[}1{]}:} \< رتب القوالب >                                                                                                                                                                                                      \\
\textbf{{[}2{]}:} \< اختبر كل خلاياك >                                                                                                                                                                                                  \\
\textbf{{[}3{]}:} \< نسق بياناتك >                                                                                                                                                                                                      \\
\textbf{{[}4{]}:} \< كن مبتكرًا >                                                                                                                                                                                                     \\
\textbf{Answer:}                                                                                                                                                                                                                   \\ \hline
\end{tabular}
\caption{Example of one-shot prompt for \textbf{ArSWAG}.} \label{tab:arswag_prompt}
\end{table*}


\subsubsection{Results}

\input{Tables/commonsense_inference}

The results are shown in Table~\ref{tab:arswag_result}. 
%We see AraGPT3 achieves significant improvements compared to in all 3 settings, with our zero-shot performance surpassing few-shot for GPT-3. Although moving from zero-shot to one-shot doesn’t improve performance much (in fact, it decreases it in this case), but including more examples in the few-shot setting substantially increases performance.

==> dialectal_JASMINE.tex <==
\section{JASMINE's Dialectal Generation}\label{sec:diaJASMINE}

\noindent\textbf{\hl{Dialectal Generation.}}  \hl{We study the quality of}~\ourmodel~\hl{dialectal output in the zero-shot setting. For this, we seed our model using  a new country-level Arabic dataset to seed our models. We explain these here.}
% \noindent\textbf{DiaGen.} We sample long sentences from each of the $25$ cities in the MADAR  dataset~\cite{bouamor2018madar} ($100$ sentences from each city).\footnote{MADAR is a 25-city multi-dialect parallel corpus in the travel domain. We extract only sentences longer than $12$ words.} We prompt ~\ourmodel\textsubscript{2.7B} with the first ten words from each of the $2,500$ sentences to acquire generated texts. Table~\ref{tab:dialects_examples} shows samples from these dialect-prompted generations, which we refer to as \textbf{DiaGen}. 
\hl{First, we use YouTube to collect Arabic series from five Arabic countries: \textit{Algeria}, \textit{Egypt}, \textit{Jordan}, \textit{Morocco}, and \textit{Yemen}.  } \hl{Then, we ask five native speakers from these countries  to transcribe segments of length $30$ seconds extracted from the collected data. We sample $100$ transcriptions from each of the five countries. Then, we seed~}\ourmodel\textsubscript{2.7B}  \hl{with them to acquire $500$ outputs. We refer to these outputs seeds by speech transcriptions as \textbf{STGen}. } Table~\ref{tab:dialects_examples} shows samples from these dialect-prompted generations.


\hl{\noindent\textbf{Human annotation.} We use STGen in two ways. First, to evaluate the ability of our}~\ourmodel\textsubscript{2.7B}  \hl{to generate  dialectal continuation. Second, to investigate whether STGen are actually from the same dialect of the prompt. For this purpose, we set a simple annotation task where we ask native speakers from $5$ Arabic countries two questions: (i)  \textit{Is the generated text MSA or dialectal}? (ii) \textit{If the generated text is dialectal, does it represent a dialect from your country?} We give each annotator data generated with prompts from their own country.}  Table~\ref{tab:dialects_examples} (Appendix~\ref{app:autocompletion}) provides generated samples from our \ourmodel\textsubscript{2.7B} with seeds from each dialect. \textcolor{blue}{I updated the previous section --Moatez.}

\noindent\textbf{Results.} \textcolor{brown}{The annotation shows the model is able to generate dialectical Arabic on average $50.43$\% on the zero-shot setting with an initial prompt from a particular dialect. The model generates Egyptian, Jordanian, Moroccan, Yemen, and Algerian dialects on average of $79,35$\%, $47,62$\%,$48,39$\%,$4,35$\%,$47.17$\% respectively.}


%\subsection{JASMINE for Data Augmentation}\label{subsec:jasmineDataAug}

%\subsection{JASMINE's Dialectal Generation}\label{subsec:jasmineDiaGen}

% In section we study the ability of JASMIN to generate the different varieties of Arabic dialects. We use the MADAR  \cite{bouamor2018madar}, a 25-city multi-dialect parallel corpus in the travel domain. We extract $100$ long dialectal sentences\footnote{Sentences that have more than $10$ words} from each dialect in MADAR corpus. Then, we use the first ten words to promote our $2.7$B model.     

==> long_lit.tex <==

\section{Related Work}\label{sec:lit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Large Language Models (LLMs).}  ~\newcite{brown2020language} developed GPT-3 and showed through extensive evaluation its abilities on few-shot learning. Several other works followed, usually with big industry labs introducing larger models~\cite{rae2021scaling,thoppilan2022lamda,smith2022using}. By way of examples, PaLM~\cite{chowdhery2022palm} is a $540$B densely activated, autoregressive Transformer language model trained on $780$B tokens.~\newcite{chowdhery2022palm} demonstrate continued benefits of scaling by achieving SOTA few-shot learning results on hundreds of NLU and NLG tasks. The model also shows strong capabilities in multilingual tasks and source code generation.~\newcite{zhang2022opt} introduce OPT and seeks to enable reproducible and responsible research at scale, and to bring more voices to the table in studying the impact of these LLMs.~\newcite{smith2022using} train Megatron-Turing NLG with 530B parameters. A number of recent works such as T0~\cite{sanh2021multitask} and FLAN~\cite{wei2021finetuned} focus on directly improving language model's zero-shot learning capabilities through large-scale multitask finetuning. BLOOM~\cite{scao2022bloom} is pretrained on a large dataset of $46$ natural and $13$ programming languages and is reported to perform competitively on a wide variety of benchmarks. It also achieves stronger results after undergoing multitask prompted finetuning.

\noindent\textbf{Behavior of LLMs.} Several works have focused on studying the behavior of large language models (LLMs). For example,~\newcite{brown2020language} find `relatively' smooth scaling for most tasks with model capacity across three different settings settings. One pattern they find is that the gap between zero-, one-, and few-shot performance often grows with model capacity. They cautiously conclude that this suggests that larger models are more proficient meta-learners. 

\noindent\textbf{Emergent Abilities of Language Models.} ~\newcite{wei2022emergent} study \textit{emergent abilities}  of language models, abilities that are not present in smaller-scale models but are present in large-scale models. For example, they find that the ability to perform a task via few-shot prompting is emergent. Other emergent examples they found include transliterating from the International Phonetic Alphabet, recovering a word from its scrambled letters, and Persian question-answering. Other intriguing capabilities exhibited by LLMs include free-form generation of coherent, long-form text (e.g., news stories), generating responses with real-world knowledge, and performing rudimentary mathematical operations~\cite{smith2022using}.

\noindent\textbf{Language Model Alignment.} Several works have studied on making the language models aligned with the human expectation.~\newcite{ziegler_summ, stiennon_summ, wu_summ} apply reinforcement learning to align language model for text summarization. Similarly, human feedback has been used to align language models for dialogue generation~\cite{jaques_dialogue, hancock_dialogue}, story generation~\cite{zhou_story}, evidence extraction~\cite{perez_evidence}. Most recently,~\newcite{madaan_gpt3} use written human feedback to augment prompts and improve the performance of GPT-3. ~\newcite{glaese_sparrow} introduce \textit{Sparrow}, an information-seeking dialogue agent trained using reinforcement learning with human feedback to be more helpful, correct, and harmless compared to prompted language models. ~\newcite{ouyang_instructgpt} develop \textit{InstructGPT}, which is finetuned using reinforcement learning to align with human intent. The finetuned model shows improvements in truthfulness and reductions in toxic output generation.

\noindent\textbf{Bias in Language Models.}
The recent success of LLMs is associated with various potential risks since the web pretraining datasets themselves are biased~\cite{bender_parrots,bommasani_risks,arteaga_bias,dodge_corpora}.%The unsupervised web text data often contains social stereotypes and biases which models can learn during the pretraining~\cite{arteaga_bias,dodge_corpora}.
~\newcite{magar_contamination, tal_gender} show that the risk of biases gets higher with the increase of the model size. As a result, these stereotypes and biases resurface during the downstream tasks, such as natural language inference (NLI)~\cite{poliak_nli, sharma_nli}, coreference resolution~\cite{rudinger_coref, zhao_coref}, and machine translation~\cite{stanovsky_mt}.

\noindent\textbf{Ethical Considerations for Language Models.} Other than bias, there are a number of other ethical considerations that have been considered for language models. These include memorizing and revealing private information~\cite{carlini_memorization}, or spreading misinformation and other malicious abuses caused by the language models~\cite{weidinger_harm}.

\noindent\textbf{Domain-Specific Language Models.}~\newcite{taylor_galactica} develop Galactica, a large language model that can store, combine, and reason about scientific knowledge.~\newcite{beltagy_scibert} propose SciBERT which is pretrained on curated scientific publications. PubMedBERT~\cite{gu_pubmedbert} and BioBERT~\cite{lee_biobert} are BERT-based models pretrained exclusively on the biomedical domain.~\newcite{chalkidis_legalbert} propose LEGAL-BERT, a domain specialized BERT pretrained on the legal domain. Besides, transformers have widely been used to learn representations of protein sequence~\cite{honda_smiles,irwin_chemformer,rives_biological,nijkamp_progen2,lin_proteinlm}.

% BIAS in LMs
%%%%%%%%%%%%%%%%
% In addition to these works, there is a growing body of literature on studying biases in language models~\cite{nadeem2021stereoset}. 

% Jurassic-1~\cite{lieber2021jurassic} % https://sharir.org/papers/jurassic_white_paper.pdf

% \textcolor{red}{The effectiveness of this method was further enhanced by recent model adaptation work such as prompt tun- ing [33], which efficiently adapts large language models to individual tasks with robust task performance. 



% \textcolor{red}{GPT-3 paper: In general, we find relatively smooth scaling for most tasks with model capacity in all three settings; one notable pattern is that the gap between zero-, one-, and few-shot performance often grows with model capacity, perhaps suggesting that larger models are more proficient meta-learners.}

% \url{https://proceedings.neurips.cc/paper/2020/file/1457c0d6bfcb4967418bfb8ac142f64a-Paper.pdf}

% \textcolor{red}{performs competitively on lan- guage tasks using in-context learning without fine-tuning or gradient updates. Such in-context learning allows models to perform new language tasks with only simple instructions and a few optional examples. The effectiveness of this method was further enhanced by recent model adaptation work such as prompt tun- ing [33], which efficiently adapts large language models to individual tasks with robust task performance. Other intriguing capabilities exhibited by large language models include, but are not limited to, free-form generation of coherent, long-form text like news stories, generating responses with real-world knowledge, as well as performing rudimentary mathematical operations.
% } 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textcolor{red}{ This is the ``Megatron-Turing NLG" paper: https://arxiv.org/pdf/2201.11990.pdf. There are some good insights in this paper. For example, which tasks to evaluate on, how to perform analysis of social biases, and also how to preprocess and deduplicate data. \url{https://arxiv.org/pdf/2201.11990.pdf}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\textcolor{red}{PaLM: ~\newcite{chowdhery2022palm}. To further our understanding of the impact of scale on few-shot learning, we trained a 540-billion parameter, densely activated, Transformer language model, which we call Pathways Language Model (PaLM). We demonstrate continued benefits of scaling by achieving state-of- the-art few-shot learning results on hundreds of language understanding and generation benchmarks. On a number of these tasks, PaLM 540B achieves breakthrough performance, outperforming the finetuned state- of-the-art on a suite of multi-step reasoning tasks, and outperforming average human performance on the recently released BIG-bench benchmark. A significant number of BIG-bench tasks showed discontinuous improvements from model scale, meaning that performance steeply increased as we scaled to our largest model. PaLM also has strong capabilities in multilingual tasks and source code generation, which we demonstrate on a wide array of benchmarks. We additionally provide a comprehensive analysis on bias and toxicity, and study the extent of training data memorization with respect to model scale. Finally, we discuss the ethical considerations related to large language models and discuss potential mitigation strategies. \url{https://arxiv.org/pdf/2204.02311.pdf}}



% Emergent Abilities of Large Language Models \url{https://arxiv.org/pdf/2206.07682.pdf}

%\textcolor{red}{~\newcite{zhang2022opt} introduce OPT and seeks to enable reproducible and responsible research at scale, and to bring more voices to the table in studying the impact of these LLMs. ~\citenew{smith2022using} train Megatron-Turing NLG with 530B parameters. % \url{"Megatron-Turing NLG}.}

% \textcolor{red}{{\bf For LIT REVIEW:} There has also been recent work focusing on directly improving language model’s zero-shot learning ca- pabilities through large-scale multitask finetuning. Both T0 [59] and FLAN [70] have taken this path and have shown that such an approach can improve zero-shot learning capabilities of language models. This approach has been shown to apply well to a pretrained language model [70], observing that the larger the model size, the more benefit it extracts from such training methods. We hope that our breakthroughs in large-scale pretraining are synergistic with these methods, and will produce even better models in the future. \url{https://arxiv.org/pdf/2201.11990.pdf}}

==> to_remove.tex <==
Thanks so much for your review and valuable comments. 

\textbf{Questions A.} Will the developed evaluation benchmarks be made available to others in the community to verify and evaluate similar models?

\textbf{Answer A.}  We emphasize that we will make all the developed evaluation benchmarks available to the community. We thank the reviewer for asking.
